Joint Learning of Assignment and Representation for Biometric Group Membership

This paper proposes a framework for group membership protocols preventing the curious but honest server from reconstructing the enrolled biometric signatures and inferring the identity of querying clients. This framework learns the embedding parameters, group representations and assignments simultaneously. Experiments show the trade-off between security/privacy and verification/identification performances.

==> relatedWork.tex <==
% !TEX root = ms.tex

\section{Related Work}
\label{sec:RelatedWorks}
